Accountability and Forensics in Blockchains: XDC Consensus Engine DPoS 2.0

This document introduces XinFin DPoS 2.0, the proposed next generation decentralized consensus engine for the XinFin XDC Network. Built upon the most advanced BFT consensus protocol, this upgrade will empower the XDC Network with military-grade security and performance while consuming extremely low resources, and will be fully backwards-compatible in terms of APIs. It will also pave the road to the future evolution of the XDC Network. The core invention is the holistic integration of accountability and forensics in blockchains: the ability to identify malicious actors with cryptographic integrity directly from the blockchain records, incorporating the latest peer-reviewed academic research with state of the art engineering designs and implementation plans.

==> forensics.tex <==
\paragraph{Safety Violation and Forensic Support}
When the adversary corrupts more than 1/3 master nodes, they can vote for two conflicting blocks within a round. Denote the two blocks as $B$ and $B'$. Let us split 2/3 honest master nodes into two sets $P$ and $Q$. If the leader is also corrupted, it can equivocate to master nodes in $P$ and $Q$. As a result, master nodes in $P$ vote for $B$ and master nodes in $Q$ vote for $B'$. Two conflicting blocks thus both get $t_H=\left \lceil{\texttt{VALIDATOR\_SET\_SIZE}\times 2/3}\right \rceil$ votes, which are enough to form two conflicting QCs within a round.

The adversary can also create a safety violation across rounds. When the adversary corrupts more than 1/3 master nodes, these master nodes can vote for a conflicting block $B'$ despite having a lock block $B$ ($B$ is not an ancestor of $B'$). Again, let us split 2/3 honest master nodes into two sets $P$ and $Q$. Master nodes in $P$ vote for $B$ in round $r$ and also lock on the QC contained in $B$'s parent block, whereas master nodes in $Q$ are not aware of that lock. Then in some higher round, a leader may propose an outdated QC with a conflicting block $B'$. Master nodes in $Q$ are not aware of the previous lock so they can vote for $B'$ along with the corrupted master nodes (and violate the voting rule). As a result, the leader can collect $t_H$ votes to form a QC in the higher round. This QC is sufficient to unlock any honest master node and subsequently they can finalize a conflicting block.

In the above examples of safety violation, we observe that the corrupted master nodes must send certain messages in order to break safety: 1) to break safety within a round, corrupted master nodes vote for two conflicting blocks in the round, 2) to break safety across rounds, they vote for a conflicting block despite having a lock on a different block (thus violating the voting rule). Those messages are signed by their secret keys hence can serve as irrefutable evidence of their misbehavior. In addition, no honest master node will vote twice within a round or violate the voting rule, therefore we will only hold corrupted master nodes culpable. Those messages are embedded into the blockchain, so by querying master nodes for conflicting blockchains, we can provide the forensic support property defined as follows.

We propose the \textit{forensic support} property, whose goal is to (i) identify as many Byzantine (corrupted) master nodes as possible, (ii) while having a large number of witnesses, and (iii) obtain the proof from querying as few witnesses as possible. There are $\texttt{VALIDATOR\_SET\_SIZE}=108$ master nodes in the system. The process of identifying culpable Byzantine master nodes involve performing appropriate quorum intersections: since two quorums of $t_H$ master nodes intersect in at least $\texttt{VALIDATOR\_SET\_SIZE}/3$ master nodes, we are able to identify that many Byzantine master nodes. As for the witnesses, two honest nodes having access to one of the two conflicting blockchains, respectively, are witnesses. Since non-master nodes also passively monitors the blockchain, they can serve as witnesses as well. This also implies that as long as there are at least two honest nodes in the XinFin network and the adversary wants to create a safety violation for the two nodes, we can provide forensic support. %So safety forensic support holds if no more than $\texttt{VALIDATOR\_SET\_SIZE}-2$ master nodes are corrupted.

We have a protocol to provide safety forensic support for the HotStuff protocol:

We take two conflicting blockchains, which diverge from some common block as shown in Figure~\ref{}, as input. \gerui{Scan the two chains to find QC? Pseudocode is better?}
If two QCs are within a round, the master nodes who vote for both QCs are corrupted master nodes.
If two QCs are across rounds, we denote by QC1 the lower one and QC2 the higher one. We scan the two chains for a QC (denoted by QC\#) such that it is later than QC1, the block $B'$ QC\# pointed to conflicts with the block $B$ that QC1 pointed to, and the QC contained in $B'$ is no later than QC1 in rounds. The master nodes who vote for QC1 and QC\# are corrupted master nodes.

Figure~\ref{} shows an example attack which results in two conflicting blockchains. TODO.

\paragraph{Liveness Violation and Forensic Support}
\gerui{something similar to slashing}

\paragraph{Implementation}
We plan to implement the corresponding forensic support protocol as a module on top of the HotStuff protocol. There is a reference implementation on top of an open source {\sf Diem} client which adopts a variant of the HotStuff protocol~\cite{}. We borrow the innovations of the reference implementation to that of the XDPoS HotStuff protocol and highlight our implementation plan as follows.

%\paragraph{Forensic module.} 
The module should consist of two components, a database \fs used to store quorum certificates received by nodes, which can be accessed by clients through some kind of requests such as RPC; and an independent \detector run by any clients who want to have safety forensic support, to analyze the forensic information. 
\begin{itemize}
    \item \textbf{\fs} maintains a map from the round number to quorum certificates and its persistent storage.
    It is responsible for storing forensic information and allows access by other components, 
    including clients (e.g., via RPC requests).  
    \item \textbf{\detector } is run by clients manually to send requests periodically to connected nodes. It collates information received from nodes, using it as the  input to the forensic support protocol.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/diem.pdf}
    \caption{Forensic module plan TODO.}
    \label{fig:forensic_store}
\end{figure}

% \paragraph{Testing using Twins~\cite{bano2020twins}.}
% To test the correctness of forensic protocols, we build a testbed to simulate Byzantine attacks and construct different types of safety violations. Ideally, for modularity purposes, our testbed should not require us to modify the underlying consensus protocol to obtain Byzantine behavior. We leverage Twins~\cite{bano2020twins}, an approach to emulate Byzantine behaviors by running two instances of a node (i.e. replica) with the same identity. Consider a simple example setting with four nodes (denoted by $node0\sim 3$), where $node0$ and $node1$ are Byzantine so they have twins called $twin0$ and $twin1$. The network is split into two partitions, the first partition $P_1$ includes nodes $\{node0, node1, node2\}$ and the second partition $P_2$ includes nodes $\{twin0, twin1, node3\}$. Nodes in one partition can only receive the messages sent from the same partition. The double voting attack can be simulated when Byzantine leader proposes different valid blocks in the same view, and within each partition, all nodes will vote for the proposed block. The network partition is used to drop all messages sent from a set of nodes. However, it can only help construct the safety violation within the view. To construct more complicated attacks, we further improve the framework and introduce another operation called ``detailed drop'', which drops selected messages with specific types.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/demo.pdf}
    \caption{Forensic module dashboard.  }
    \label{fig:demo}
\end{figure}
%\paragraph{Visualization.} 
The \detector accepts the registration of different rounds to get notified once the data is updated. We plan to built  a dashboard to display the  information received by the detector and the analysis results output by the forensic support protocol.  Figure~\ref{fig:demo} shows a snapshot of the dashboard   which displays  information about the network topology, hashes of latest blocks received at different nodes, conflicting blocks, detected culprit keys and raw logs. 
